AGAPECert: An Auditable, Generalized, Automated, Privacy-Enabling Certification Framework with Oblivious Smart Contracts

This paper introduces AGAPECert, an Auditable, Generalized, Automated, Privacy-Enabling, Certification framework capable of performing auditable computation on private data and reporting real-time aggregate certification status without disclosing underlying private data. AGAPECert utilizes a novel mix of trusted execution environments, blockchain technologies, and a real-time graph-based API standard to provide automated, oblivious, and auditable certification. Our technique allows a privacy-conscious data owner to run pre-approved Oblivious Smart Contract code in their own environment on their own private data to produce Private Automated Certifications. These certifications are verifiable, purely functional transformations of the available data, enabling a third party to trust that the private data must have the necessary properties to produce the resulting certification. Recently, a multitude of solutions for certification and traceability in supply chains have been proposed. These often suffer from significant privacy issues because they tend to take a" shared, replicated database" approach: every node in the network has access to a copy of all relevant data and contract code to guarantee the integrity and reach consensus, even in the presence of malicious nodes. In these contexts of certifications that require global coordination, AGAPECert can include a blockchain to guarantee ordering of events, while keeping a core privacy model where private data is not shared outside of the data owner's own platform. AGAPECert contributes an open-source certification framework that can be adopted in any regulated environment to keep sensitive data private while enabling a trusted automated workflow.

==> 10_future_work.tex <==
%-------------------------------------------------------------------------------
\section{Future Work}
\label{sec:future_work}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
\subsection{Untrusted Compute Engine}
\label{ssec:untrusted_compute_engine}
%-------------------------------------------------------------------------------

AGAPECert future releases can include a different threat model; that is, an untrusted compute engine. In such a scenario, all data must be passed encrypted through the enclave exterior and only decrypted by the enclave interior. However, in an adversarial environment, data encryption is not enough to protect privacy. Access patterns can leak a significant amount of information~\cite{Stefanov2013} (contention in the data, most accessed block/shard.) We are interested in access patterns to the storage (memory, disk, cache) and over the network.  Oblivious RAM algorithms tackle this problem by hiding access patterns to the data through reshuffling and re-encrypting data as it is accessed. ORAM algorithms guarantee that an adversary has a negligible probability of learning the real access pattern to the data~\cite{Stefanov2013}. Our future work can include Path ORAM as a prominent tool to provide oblivious computation on an untrusted node (outsourced compute engine.)

